GradViT: Gradient Inversion of Vision Transformers

In this work we demonstrate the vulnerability of vision transformers (ViTs) to gradient-based inversion attacks. During this attack, the original data batch is reconstructed given model weights and the corresponding gradients. We introduce a method, named GradViT, that optimizes random noise into naturally looking images via an iterative process. The optimization objective consists of (i) a loss on matching the gradients, (ii) image prior in the form of distance to batch-normalization statistics of a pretrained CNN model, and (iii) a total variation regularization on patches to guide correct recovery locations. We propose a unique loss scheduling function to overcome local minima during optimization. We evaluate GadViT on ImageNet1K and MS-Celeb-1M datasets, and observe unprecedentedly high fidelity and closeness to the original (hidden) data. During the analysis we find that vision transformers are significantly more vulnerable than previously studied CNNs due to the presence of the attention mechanism. Our method demonstrates new state-of-the-art results for gradient inversion in both qualitative and quantitative metrics. Project page at https://gradvit.github.io/.

==> Images/block_wise.tex <==
\begin{figure}[t]
\centering

\resizebox{\linewidth}{!}{
\begingroup
\renewcommand*{\arraystretch}{0.3}
% \setlength\extrarowheight{-30pt}
\begin{tabular}{ccc}
%original
\includegraphics[width=0.45\linewidth,clip,trim=5px 0 0 4px]{Images/block_specific/img1_patch.jpg} &
\includegraphics[width=0.45\linewidth,clip,trim=5px 0 0 4px]{Images/block_specific/img2_patch.jpg} &
\includegraphics[width=0.45\linewidth,clip,trim=5px 0 0 4px]{Images/block_specific/img3_patch.jpg}
\\
\multicolumn{3}{c}{(a) Blocks 1-4 (ViT/B16) }
%deepdream
\end{tabular}
\endgroup
}

\resizebox{\linewidth}{!}{
\begingroup
\renewcommand*{\arraystretch}{0.3}
% \setlength\extrarowheight{-30pt}
\begin{tabular}{ccc}
\includegraphics[width=0.45\linewidth,clip,trim=5px 0 0 4px]{Images/block_wise/img1_layer1.jpg} &
\includegraphics[width=0.45\linewidth,clip,trim=5px 0 0 4px]{Images/block_wise/img2_layer1.jpg} &
\includegraphics[width=0.45\linewidth,clip,trim=5px 0 0 4px]{Images/block_wise/img3_layer1.jpg} \\
\multicolumn{3}{c}{(b) Blocks 5-8 (ViT/B16) }
%deepdream
\end{tabular}
\endgroup
}

\resizebox{\linewidth}{!}{
\begingroup
\renewcommand*{\arraystretch}{0.3}
% \setlength\extrarowheight{-30pt}
\begin{tabular}{ccc}
\includegraphics[width=0.45\linewidth,clip,trim=5px 0 0 4px]{Images/block_wise/img1_layer1.jpg} &
\includegraphics[width=0.45\linewidth,clip,trim=5px 0 0 4px]{Images/block_wise/img2_layer1.jpg} &
\includegraphics[width=0.45\linewidth,clip,trim=5px 0 0 4px]{Images/block_wise/img3_layer1.jpg} \\
\multicolumn{3}{c}{(c) Blocks 5-8 (ViT/B16) }
%deepdream
\end{tabular}
\endgroup
}

\resizebox{\linewidth}{!}{
\begingroup
\renewcommand*{\arraystretch}{0.3}
% \setlength\extrarowheight{-30pt}
\begin{tabular}{ccc}
\includegraphics[width=0.45\linewidth,clip,trim=5px 0 0 4px]{Images/block_wise/img1_layer1.jpg} &
\includegraphics[width=0.45\linewidth,clip,trim=5px 0 0 4px]{Images/block_wise/img2_layer1.jpg} &
\includegraphics[width=0.45\linewidth,clip,trim=5px 0 0 4px]{Images/block_wise/img3_layer1.jpg} \\
\multicolumn{3}{c}{(d) Blocks 5-8 (ViT/B16) }
%deepdream
\end{tabular}
\endgroup
}

\resizebox{\linewidth}{!}{
\begingroup
\renewcommand*{\arraystretch}{0.3}
% \setlength\extrarowheight{-30pt}
\begin{tabular}{ccc}
%original
\includegraphics[width=0.45\linewidth,clip,trim=5px 0 0 4px]{Images/block_wise/img1_layer2.jpg} &
\includegraphics[width=0.45\linewidth,clip,trim=5px 0 0 4px]{Images/block_wise/img2_layer2.jpg} &
\includegraphics[width=0.45\linewidth,clip,trim=5px 0 0 4px]{Images/block_wise/img3_layer2.jpg} \\
\multicolumn{3}{c}{(e) Blocks 9-12 (ViT/B16)}
%deepdream
\end{tabular}
\endgroup
}
\caption{Recovered images by removing the gradient contributions from various layers in the ViT/B16 architecture in InViT model. It is evident that later layers (9-12) contain the most critical information that leads to data leakage. }
\vspace{-0.5mm}
\label{fig:layerwise}
\end{figure}


























% \begin{figure}[t]
% \centering

% \resizebox{\linewidth}{!}{
% \begingroup
% \renewcommand*{\arraystretch}{0.3}
% % \setlength\extrarowheight{-30pt}
% \begin{tabular}{ccc}
% %original
% \includegraphics[width=0.45\linewidth,clip,trim=5px 0 0 4px]{figures/bs48_seed100_rank0.jpg} &
% \includegraphics[width=0.45\linewidth,clip,trim=5px 0 0 4px]{figures/bs48_images/bs48_new.jpg} &
% \includegraphics[width=0.45\linewidth,clip,trim=5px 0 0 4px]{figures/bs48_images/seed5901_rank0.jpg}
% \\
% \multicolumn{3}{c}{(a) details restored}
% %deepdream
% \end{tabular}
% \endgroup
% }

% \resizebox{\linewidth}{!}{
% \begingroup
% \renewcommand*{\arraystretch}{0.3}
% % \setlength\extrarowheight{-30pt}
% \begin{tabular}{ccc}
% \includegraphics[width=0.45\linewidth,clip,trim=5px 0 0 4px]{figures/bs48_images/seed102_rank0.jpg} &
% % \includegraphics[width=0.49\linewidth,clip,trim=5px 0 0 4px]{figures/bs48_images/seed101_rank0.jpg} &
% \includegraphics[width=0.45\linewidth,clip,trim=5px 0 0 4px]{figures/bs48_images/seed103_rank2.jpg} &
% \includegraphics[width=0.45\linewidth,clip,trim=5px 0 0 4px]{figures/bs48_images/seed100_rank0.jpg} \\
% \multicolumn{3}{c}{(b) semantics restored}
% %deepdream
% \end{tabular}
% \endgroup
% }

% \resizebox{\linewidth}{!}{
% \begingroup
% \renewcommand*{\arraystretch}{0.3}
% % \setlength\extrarowheight{-30pt}
% \begin{tabular}{ccc}
% %original
% \includegraphics[width=0.45\linewidth,clip,trim=5px 0 0 4px]{figures/bs48_images/seed5901_rank2.jpg} &
% \includegraphics[width=0.45\linewidth,clip,trim=5px 0 0 4px]{figures/bs48_images/seed100_rank4.jpg} &
% \includegraphics[width=0.45\linewidth,clip,trim=5px 0 0 4px]{figures/bs48_images/seed104_rank2.jpg} \\
% \multicolumn{3}{c}{(c) no visual information}
% %deepdream
% \end{tabular}
% \endgroup
% }
% \caption{Varying level of information leakage at batch size $48$ on ImageNet validation set. Each block containing a pair of (left) original sample and its (right) reconstruction by GradInversion. }
% \vspace{-0.5mm}
% \label{fig:bs48_imgs}
% \end{figure}


==> Images/grad_inv_fig5.tex <==
\begin{figure}[t]
\centering

\resizebox{0.75\linewidth}{!}{
\begingroup
\renewcommand*{\arraystretch}{0.3}
% \setlength\extrarowheight{-30pt}
\begin{tabular}{ccc}
%original
\includegraphics[width=0.33\linewidth,clip,trim=5px 0 0 4px]{figures/bs1_ablation/original.png} &
%ADI
\includegraphics[width=0.33\linewidth,clip,trim=5px 0 0 4px]{figures/bs1_ablation/dgl.png} &
%deepdream
\includegraphics[width=0.33\linewidth,clip,trim=5px 0 0 4px]{figures/bs1_ablation/fgi.png}
\\
Original & Zhu \etal~\cite{zhu2019deep} & Geiping \etal~\cite{geiping2020inverting}
\\
\end{tabular}
%
\endgroup
}

\resizebox{0.5\linewidth}{!}{
\begingroup
\renewcommand*{\arraystretch}{0.3}
% \setlength\extrarowheight{-30pt}
\begin{tabular}{cc}
\includegraphics[width=0.33\linewidth,clip,trim=4px 0 0 4px]{figures/bs1_ablation/ours_no_bn.png} &
\includegraphics[width=0.33\linewidth,clip,trim=5px 0 0 4px]{figures/bs1_ablation/ours_bn.png}
\\
(d) \textbf{Ours} - BN$_{\text{approx.}}$ & (e) \textbf{Ours} - BN$_{\text{exact}}$\\
\end{tabular}
\endgroup
}

\caption{Comparison with prior art on ResNet-50 (ImageNet) gradient inversion at batch size 1 for a ``challenging'' sample from~\cite{geiping2020inverting}. 
%Results of prior work based on the public repositories from the authors at~\cite{zgeiping_github,zzhu_github}. 
}
\label{fig:bs1_comparison}
\end{figure}


==> Images/grad_inv_table3.tex <==
\begin{table}[!t]
\centering
\resizebox{.78\linewidth}{!}{
\begin{tabular}{lcccc}
\toprule
\multirow{2}{*}{\textbf{Model}}  & \multicolumn{4}{c}{\textbf{Distance to Original Images}}\\
\cmidrule{2-5}
& FFT$_\text{2D}$ $\downarrow$ & PSNR $\uparrow$  & LPIPS $\downarrow$  \\
\midrule
ResNet-50 (MOCO V2)   & $0.175$ & $12.929$  & $0.484$ \\
ResNet-50 (standard)  & $0.204$ & $11.771$  & $0.584$ \\
ResNet-18 (standard)  & $0.218$ & $10.729$  & $0.693$ \\
\bottomrule
\end{tabular}}
%\textbf{CIFAR-10. }
\caption{Reconstruction under varying feature extraction strength.}
\label{tab:nomoco}
\vspace{-1mm}
\end{table}


==> Images/teaser.tex <==
\begin{strip}\centering
\includegraphics[width=\textwidth,clip]{fig/teaser.pdf}
\captionof{figure}{
We introduce DeViT, a method to enable dynamic tokens\yin{change into new teaser - this is temp. placeholder}.  
\label{fig:teaser}}
\end{strip}

% parameter server , workers 

==> sec7_protection.tex <==
\section{Protection Mechanisms}
One appealing aspect of distributed machine learning and, in particular, federated learning is the capability of training global models across many clients by only sharing gradient updates. However, in this work, we have demonstrated vulnerabilities of different models such as ViTs to data leakage by exploiting the shared gradients. Hence, it is essential to devise protection algorithms to address the growing data security concerns. We hint on potential solutions based on our extensive component-based data leakage analysis as described in Sec.~\ref{sec:data_leakage}. The first proposed solution is to leverage differential privacy methods~\cite{dwork2006calibrating,li2019privacy}. Specifically, one could add Gaussian noise to MSA blocks or the last four layers to reduce the amount of data leakage. Another potential solution is to utilize cryptographic techniques like secure multi-party computation~\cite{kaissis2020secure} or homomorphic encryption~\cite{zhang2020batchcrypt} to secure the aforementioned layers and obscure any important information embedded in the gradients. 
We believe that these techniques can be effective in protecting against GradViT.

==> tables/vit_arch_abl.tex <==
\begin{table}[!t]
\centering
\resizebox{.6\linewidth}{!}{
\begin{tabular}{lcccc}
\toprule
\multirow{2}{*}{\textbf{Network}}  & \multicolumn{4}{c}{\textbf{Image Reconstruction Metric}}\\
\cmidrule{2-5}
&PSNR $\uparrow$& FFT$_\text{2D}$ $\downarrow$  & LPIPS $\downarrow$  \\
\midrule
ViT-T/16   & $12.521$ & $0.062$ & $0.483$   \\
ViT-S/32  & $12.365$ & $0.063$ & $0.505$   \\
ViT-S/16  & $13.658$ & $0.042$ & $0.412$    \\
% ViT-L/16~\cite{DBLP:conf/iclr/DosovitskiyB0WZ21}  &- & $15.515$ & $0.076$ & $0.454$   \\
ViT-B/32 &- & $13.599$ & $0.048$ & $0.436$   \\
ViT-B/16&- & $\mathbf{15.515}$ & $\mathbf{0.032}$ & $\mathbf{0.295}$ \\
\bottomrule
\end{tabular}}
%\textbf{CIFAR-10. }
\caption{Effect of excluding layer-wise gradients on final reconstruction accuracy in ViT-B/16.}
\label{tab:abl_vit_study}
\vspace{-1mm}
\end{table}
